Undecidability of a weak version of MSO+U

We prove the undecidability of MSO on $\omega$-words extended with the second-order predicate $U_1(X)$ which says that the distance between consecutive positions in a set $X \subseteq \mathbb{N}$ is unbounded. This is achieved by showing that adding $U_1$ to MSO gives a logic with the same expressive power as $MSO+U$, a logic on $\omega$-words with undecidable satisfiability. As a corollary, we prove that MSO on $\omega$-words becomes undecidable if allowing to quantify over sets of positions that are ultimately periodic, i.e., sets $X$ such that for some positive integer $p$, ultimately either both or none of positions $x$ and $x+p$ belong to $X$.

==> edit.tex <==
%% à basculer pour virer les remarques
\newif\ifdraft\draftfalse
\newif\ifdraft\drafttrue

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdraft

\newcommand\comment[1]{}

\RequirePackage{savesym}	\savesymbol{checkmark}
\RequirePackage{dingbat}	\restoresymbol{lipics}{checkmark}
\RequirePackage{microtype}

%\DeclareUnicodeCharacter{00A0}{~}
%[gb]: j'avais un problème d'encodage, j'ai ajouté la ligne ci-dessus pour résoudre mon problème.
%      (src: http://tex.stackexchange.com/questions/83440/inputenc-error-unicode-char-u8-not-set-up-for-use-with-latex)

\definecolor{daviaudl}{rgb}{1,0,.5}
\definecolor{guillonb}{rgb}{.93,.57,.13}
\definecolor{sreejith}{rgb}{.23,.89,.13}

\newcommand{\showversion}{%
	{\footnotesize\begin{center}\textbf{Version of \today}\end{center}}%
}

\newcommand*\bgdone{\textcolor{guillonb}{$\surd$}}
\newcommand*\vpdone{\textcolor{blue}{$\surd$}}
\newcommand*\lddone{\textcolor{daviaudl}{$\surd$}}
\newcommand*\mbdone{\textcolor{purple}{$\surd$}}
\newcommand*\srdone{\textcolor{sreejith}{$\surd$}}

\newcommand*\bglike{\textcolor{guillonb}{\leftthumbsup}}
\newcommand*\vplike{\textcolor{blue}{\leftthumbsup}}
\newcommand*\ldlike{\textcolor{daviaudl}{\leftthumbsup}}
\newcommand*\mblike{\textcolor{purple}{\leftthumbsup}}
\newcommand*\srlike{\textcolor{sreejith}{\leftthumbsup}}

\newcommand*\bgdislike{\textcolor{guillonb}{\leftthumbsdown}}
\newcommand*\vpdislike{\textcolor{blue}{\leftthumbsdown}}
\newcommand*\lddislike{\textcolor{daviaudl}{\leftthumbsdown}}
\newcommand*\mbdislike{\textcolor{purple}{\leftthumbsdown}}
\newcommand*\srdislike{\textcolor{sreejith}{\leftthumbsdown}}

\newcommand\bg[1]{{\color{guillonb} [#1 --\textbf{Bruno}]}}
\newcommand\vp[1]{{\color{blue} [#1 --\textbf{Vincent}]}}
\newcommand\ld[1]{{\color{daviaudl} [#1 --\textbf{Laure}]}}
\newcommand\mb[1]{{\color{purple} [#1 --\textbf{Mikołaj}]}}
\newcommand\sr[1]{{\color{sreejith} [#1 --\textbf{Sreejith}]}}

\newcommand\bgtodo[1]{{\color{guillonb} [\textcolor{brown}{TODO:} #1]}}
\newcommand\vptodo[1]{{\color{blue} [\textcolor{brown}{TODO:} #1]}}
\newcommand\ldtodo[1]{{\color{daviaudl} [\textcolor{brown}{TODO:} #1]}}
\newcommand\mbtodo[1]{{\color{purple} [\textcolor{brown}{TODO:} #1]}}
\newcommand\srtodo[1]{{\color{sreejith} [\textcolor{brown}{TODO:} #1]}}

\newcommand\bgchanged[1]{{\color{guillonb}{#1}}}
\newcommand\vpchanged[1]{{\color{blue}{#1}}}
\newcommand\ldchanged[1]{{\color{daviaudl}{#1}}}
\newcommand\mbchanged[1]{{\color{purple}{#1}}}
\newcommand\srchanged[1]{{\color{sreejith}{#1}}}

\newcommand*\bgsection[1][]{\textcolor{guillonb}{\newline\noindent [#1]\hrulefill\linebreak\indent}}
\newcommand*\vpsection[1][]{\textcolor{blue}{\newline\noindent [#1]\hrulefill\linebreak\indent}}
\newcommand*\ldsection[1][]{\textcolor{daviaudl}{\newline\noindent [#1]\hrulefill\linebreak\indent}}
\newcommand*\mbsection[1][]{\textcolor{purple}{\newline\noindent [#1]\hrulefill\linebreak\indent}}
\newcommand*\srsection[1][]{\textcolor{sreejith}{\newline\noindent [#1]\hrulefill\linebreak\indent}}

\newenvironment{outline}{\color{green!70!black}\begin{itemize}}{\end{itemize}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\else

\newcommand\showversion{}
%\newcommand\review[1]{}

\newcommand\bg[1]{}\newcommand*\bglike{}\newcommand*\bgdislike{}\newcommand*\bgdone{}\newcommand*\bgchanged[1]{#1}\newcommand*\bgsection[1][]{}
\newcommand\vp[1]{}\newcommand*\vplike{}\newcommand*\vpdislike{}\newcommand*\vpdone{}\newcommand*\vpchanged[1]{#1}\newcommand*\vpsection[1][]{}
\newcommand\ld[1]{}\newcommand*\ldlike{}\newcommand*\lddislike{}\newcommand*\lddone{}\newcommand*\ldchanged[1]{#1}\newcommand*\ldsection[1][]{}
\newcommand\mb[1]{}\newcommand*\mblike{}\newcommand*\mbdislike{}\newcommand*\mbdone{}\newcommand*\mbchanged[1]{#1}\newcommand*\mbsection[1][]{}
\newcommand\sr[1]{}\newcommand*\srlike{}\newcommand*\srdislike{}\newcommand*\srdone{}\newcommand*\srchanged[1]{#1}\newcommand*\srsection[1][]{}

\newenvironment{outline}{\begin{comment}}{\end{comment}}

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

